LUCON: Data Flow Control for Message-Based IoT Systems

Today's emerging Industrial Internet of Things (IIoT) scenarios are characterized by the exchange of data between services across enterprises. Traditional access and usage control mechanisms are only able to determine if data may be used by a subject, but lack an understanding of how it may be used. The ability to control the way how data is processed is however crucial for enterprises to guarantee (and provide evidence of) compliant processing of critical data, as well as for users who need to control if their private data may be analyzed or linked with additional information - a major concern in IoT applications processing personal information. In this paper, we introduce LUCON, a data-centric security policy framework for distributed systems that considers data flows by controlling how messages may be routed across services and how they are combined and processed. LUCON policies prevent information leaks, bind data usage to obligations, and enforce data flows across services. Policy enforcement is based on a dynamic taint analysis at runtime and an upfront static verification of message routes against policies. We discuss the semantics of these two complementing enforcement models and illustrate how LUCON policies are compiled from a simple policy language into a first-order logic representation. We demonstrate the practical application of LUCON in a real-world IoT middleware and discuss its integration into Apache Camel. Finally, we evaluate the runtime impact of LUCON and discuss performance and scalability aspects.

==> figures/example-flow <==

\usetikzlibrary{arrows,automata}
\usetikzlibrary{shadows}
\usetikzlibrary{positioning}

\makeatletter
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ââflipped pageââ
\pgf@xc=\pgf@xb \advance\pgf@xc by-12.5pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-12.5pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother
\tikzset{
    state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=2em,
           inner sep=5pt,
           text centered,
           },
    message/.style={
           document,
			fill=white,
			line width=1pt,
           inner sep=5pt,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
}

\begin{tikzpicture}[->,>=stealth']

 % Position of QUERY 
 % Use previously defined 'state' as layout (see above)
 % use tabular for content to get columns/rows
 % parbox to limit width of the listing
 \node[message] (MESSAGE) 
 {\begin{tabular}{l}
  \textbf{Message $m$}\\
  ~\\
  \parbox{5.5cm}{
	$L_m=\{personal,health\}$\\
	$P=\{publish \leftarrow \neg personal\}$\\
  }
 \end{tabular}};
  
 % State: SERVICE_A 
 \node[state,    	% layout (defined above)
  yshift=0cm, 		% move 2cm in y
  below of=MESSAGE, 	% Position is to the right of MESSAGE
  node distance=4cm, 	% distance to MESSAGE
  anchor=center] (SERVICE_A) 	% posistion relative to the center of the 'box'
 {%
 \begin{tabular}{l} 	% content
	\textbf{Service A}\\
	(Database)\\
	~\\
	\parbox{5.5cm}{
	\begin{equation}
	\begin{aligned}
		$T^- = \emptyset$\\
		$T^- = \emptyset$\\
		$A = \{persist(\texttt{hdfs2://...}),\\ delete(\texttt{30 days})\}$
	\end{aligned}
	\end{equation}
	}
 \end{tabular}
 };
 
 % STATE SERVICE_B
 \node[state,
  right of=SERVICE_A,
  node distance=7cm,
  anchor=center] (SERVICE_B) 
 {%
 \begin{tabular}{l}
	\textbf{Service B}\\
	(Anonymizer)\\
	~\\
	\parbox{4.5cm}{
		$T^ -=\{personal\}$\\
		$T^+=\emptyset$\\
		$A = \emptyset$
	}
 \end{tabular}
 };

 % STATE SERVICE_C
 \node[state,
  right of=SERVICE_B,
  node distance=7cm,
  anchor=center] (SERVICE_C) 
 {%
 \begin{tabular}{l}
	\textbf{Service C}\\
    (Publisher)\\
	~\\
	  \parbox{5.5cm}{
			$T^-=\emptyset$\\
			$T^+=\emptyset$\\
			$A = \{publish(\texttt{http://...})\}$
		}
 \end{tabular}
 };

 % draw the paths and and print some Text below/above the graph
 \path 	(MESSAGE) 	edge  node[anchor=west,left]{$SC_n=0$}   (SERVICE_A)
			 (SERVICE_A)		   	edge																(SERVICE_B)
			 (SERVICE_B)		   	edge																(SERVICE_C)
;

\end{tikzpicture}
\end{document}

